Sales Policies for a Virtual Assistant

We study the implications of selling through a voice-based virtual assistant (VA). The seller has a set of products available and the VA decides which product to offer and at what price, seeking to maximize its revenue, consumer- or total-surplus. The consumer is impatient and rational, seeking to maximize her expected utility given the information available to her. The VA selects products based on the consumer's request and other information available to it and then presents them sequentially. Once a product is presented and priced, the consumer evaluates it and decides whether to make a purchase. The consumer's valuation of each product comprises a pre-evaluation value, which is common knowledge, and a post-evaluation component which is private to the consumer. We solve for the equilibria and develop efficient algorithms for implementing the solution. We examine the effects of information asymmetry on the outcomes and study how incentive misalignment depends on the distribution of private valuations. We find that monotone rankings are optimal in the cases of a highly patient or impatient consumer and provide a good approximation for other levels of patience. The relationship between products' expected valuations and prices depends on the consumer's patience level and is monotone increasing (decreasing) when the consumer is highly impatient (patient). Also, the seller's share of total surplus decreases in the amount of private information. We compare the VA to a traditional web-based interface, where multiple products are presented simultaneously on each page. We find that within a page, the higher-value products are priced lower than the lower-value products when the private valuations are exponentially distributed. Finally, the web-based interface generally achieves higher profits for the seller than a VA due to the greater commitment power inherent in its presentation.

==> app3_algorithm.tex <==
\section{Algorithm}\label{app_algorithm}
The algorithm can be formally described as follows. \\
\begin{algorithm}[H] \label{alg_GPS}
\KwIn{\\An array $\{(v_i,c_i)\}_{i=1}^n$ of length $n$ that specifies the observable valuation/ cost of each product. \\Initially, set $\bsigma = (1,\cdots, n), V_{opt}= V^s(\bsigma) (V^p(\bsigma)), \text{Imp}=1$}
\KwOut{\\The optimal ranking and surplus $[\bsigma, V_{opt}]$\\}
\While{\text{Imp}=1}{
    $[\bsigma', V'] = \max_{\bsigma' \in\vR(\bsigma)} V^s(\bsigma') (V^p(\bsigma')) $\;
    \eIf{$V'> V_{opt}$}{
        $V_{opt}\leftarrow V',\bsigma \leftarrow \bsigma' $\;
        Imp$=1$\;
    }{    Imp$=0$\;
}
    }
\caption{Greedy Pairwise-Switch (GPS) Algorithm}
\end{algorithm}
\noindent
%From section \ref{pf_thm_equivsln}, we know that the objective function is quasiconvex in its decision variable. Notice that the GPS algorithm essentially checks the local optimality of the proposed order and then the global optimality follows from the quasiconvexity.



==> parking lot/app4_num_products.tex <==

\subsubsection{Expected number of products searched}
The number of products viewed is another important performance measure. As the variance increases, the matching probability decreases but the product price also decreases. This two factors have opposite effects on the number of products consumer viewed. As $k$ increases, the number of product per page increases but the probability of purchase may decrease. It is unclear which of two factors dominate in reality. Moreover, the comparison in two interface is unclear at the first glance since the matching probability in each stage doesn't have a monotonic relation.\\
For web interface, the expected number of products searched is increasing in $k$. First of all, as the number of products displayed per page increases, the consumer knows that it's more likely that there are better options in the next page, in other words, their optimal threshold increase, which makes them reluctant to purchase at the early pages, and shifts the purchase probability towards the end of selling season. Therefore, in expectation, they view more products. Another reason behind this phenomena is that as the number increases, the platform has more market power from within page price commitment. It ranks the product so that the most favored products are presented in the last few pages, which also increases the number of products viewed by a consumer. \\
For both virtual assistant and web interface, the expected number of products searched is increasing in the shape parameter $a$ and increasing in the consumer survival probability $\rho$. The trend can also be explained by the reasons provided above.\\
For the comparison between the web interface and a virtual assistant, the consumer always views less product in the virtual assistant. The difference between two platforms increases as the consumer becomes more patient. Interestingly, this result is independent of the problem parameters and holds in the case when purchase probability is higher in a virtual assistant. 
    
    \begin{figure}[!htbp]
    \centering
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho10_k2_n3.png}}
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho10_k3_n2.png}}
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho10_k6_n1.png}}\\
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho99_k2_n3.png}}
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho99_k3_n2.png}}
    \subfloat[ ]{\includegraphics[width=0.32\textwidth]{web_vs_va/Eprdts_rho99_k6_n1.png}}
    \caption{Expected number of product searched.}
    \label{webvsva_Eprdts}
    \end{figure}          
     


==> parking lot/probabolistic_relax.tex <==

\subsection{Probabilistic relaxation}
The model introduced above can be reformulated as an integer programming problem: 
\eqss{
\max_Q & ~V^s (V^p) \\
\St  & \sum_i Q_{ij}=1, \forall j = 1, \cdots,n,  \\
& \sum_j Q_{ij}=1, \forall i = 1, \cdots,n,\text{ and} \\
& Q_{ij} \in \{0,1\},
}
where $  Q_{ij} =1$ if and only if product $i$ is presented in period $j.$ The matrix $Q$ is doubly stochastic. If we relax the integer constraint and still impose the doubly stochastic constraint on $Q,$ the resulting problem provides an upperbound for the original problem. We call this model ``relaxed probabilistic model (RPM)''.
\eqss{
\max_Q & ~V^s (V^p)\\
\St & \sum_i Q_{ij}=1,  \forall j = 1, \cdots,n, \\
& \sum_j Q_{ij}=1, \forall i = 1, \cdots,n,\text{ and} \\
& Q_{ij} \in [0,1]
}
\noindent
Next, we show that RPM not only provides an upperbound on the value achieved but in fact provides the optimal solution.
\begin{thm}{\emph{\textbf{(Model equivalence).}}}
\label{thm_equivsln} For the altruistic and profit-maximizing platform, the solution of the relaxed probabilistic model gives the optimal ranking.
\end{thm}
\textbf{Outline of Proof.}\\
The proof of theorem \ref{thm_equivsln} consists of the following steps: 
\begin{itemize}
    \item step 1: the scheme to calculate $V^s(Q) (V^p(Q))$ is the same in both models
    \item step 2: the feasible set $\cA$ of PM is convex and its extreme points are integer-valued.
    \item step 3 (not proved): the objective function $V^s(Q) (V^p(Q))$ is quasiconvex in the variables of $ \bar{\vM}:= Q \vM$, where $\vM$ is a constant vector.
    \item step 4: combine step 2 and step 3, the optimal solution of PM is integer-valued. Therefore, the optimal solution of the original model coincides with PM.
\end{itemize}
Notice that Theorem \ref{thm_equivsln} shows that the optimal solution of RPM can be found at its extreme points. Following the same proof as the Simplex method of linear programming, We can show the optimality of the GPS algorithm. The (incomplete) proof can be found in appendix \ref{pf_thm_equivsln}. Importantly, we still have the gap in the proof whereas we need to show that the objective function is quasiconvex in the decision variable. The heuristic is true in large number of exhaustive numerical simulations. 

==> parking lot/surplusRatio_patience.tex <==
\subsubsection{Consumer patience level (profit-maximizing platform)} \label{subsec:va_patience}
We use Gamma distribution to illustrate the effect of consumer patience level on the surplus allocation for a profit-maximizing platform. In the numerical experiment, we fix the mean $\EE(\epsilon) = 1$, set $a \in \{0.5, 2\}$, and vary $\rho \in \{0.1, 0.4, 0.7, 1\}$. We examine the effect when information asymmetry is either high ($a = 0.5$) or low ($a = 2$).
\begin{figure}[!htbp]
    \centering
    \includegraphics[width= 0.6\textwidth]{pic/pshare_patiencea123.png}
    \caption{Platform surplus share for a profit-maximizing virtual assistant platform. \commwb{What}}
    \label{webvsva_surplusallocation}
    \end{figure}

==> sec6_other_objectives.tex <==
\section{Other objective functions and surplus allocation}
\label{sec_other_obj}
In this section, we consider a virtual assistant (web-interface) of different objective functions. Specifically, we consider,
\begin{itemize}
    \item an altruistic platform that maximizes the total surplus, and
    \item a consumer agent that maximizes the consumer surplus.
\end{itemize}
Formally, an altruistic platform/ consumer agent maximizes the following objective.

\begin{align*}
\label{eq:def_eqm_apca}
\text{For an altruistic platform, }(\bsigma,\vp) & = \argmax_{(\bm{\delta},\bm{p})} \EE[V^p(\bm{\delta},\bsigma,\bm{p})+ V^c(\bm{\delta},\bsigma,\bm{p})] \\ 
\text{For a consumer agent, }(\bsigma,\vp) & = \argmax_{(\bm{\delta},\bm{p})} \EE[V^c(\bm{\delta},\bsigma,\bm{p})] 
\end{align*}

We study the platform performance under different objective functions and investigate how the comparison (between the virtual assistant and web-interface) depending on different objective functions. 

\subsection{Optimal pricing}
We first study the optimal pricing for a different objective functions. Note that virtual assistant is a special case of the web-interface by setting the number of product per page $k=1$. 

\begin{prop}{\emph{\textbf{(Altruistic platform: optimal price for  $\epsilon \sim F(\cdot)$).}}}\label{prop:ap_pricing}
Assume the support of $F(\cdot)$ is positive. The optimal price of products equals the cost: $ p_i = c_i$.
\end{prop}

\begin{prop}{\emph{\textbf{(Consumer agent: optimal price for  $\epsilon \sim F(\cdot)$).}}}\label{prop:ca_pricing}
Assume the support of $F(\cdot)$ is positive and the platform may not subsidize the consumer, i.e., $ p_i \geq c_i$. The optimal price of products equals the cost: $ p_i = c_i$.
\end{prop}

From \cite{}

% \subsection{Numerical experiments}
% 6 pics with $N=6$, $\rho = \{0.1, 1\}, \kappa = [1,k], k = [1, 2,3,6]$.
% \subsection{Consumer agent}
% 6 pics with $N=6$, $\rho = \{0.1, 1\}, \kappa = [1,k], k = [1, 2, 3, 6], Gamma(a, b) ab = 1, a = 1: 0.5 : 3$.





